Large-Scale Generative Data-Free Distillation

Knowledge distillation is one of the most popular and effective techniques for knowledge transfer, model compression and semi-supervised learning. Most existing distillation approaches require the access to original or augmented training samples. But this can be problematic in practice due to privacy, proprietary and availability concerns. Recent work has put forward some methods to tackle this problem, but they are either highly time-consuming or unable to scale to large datasets. To this end, we propose a new method to train a generative image model by leveraging the intrinsic normalization layers' statistics of the trained teacher network. This enables us to build an ensemble of generators without training data that can efficiently produce substitute inputs for subsequent distillation. The proposed method pushes forward the data-free distillation performance on CIFAR-10 and CIFAR-100 to 95.02% and 77.02% respectively. Furthermore, we are able to scale it to ImageNet dataset, which to the best of our knowledge, has never been done using generative models in a data-free setting.

==> sections/related-work-previous.tex <==
\section{Related Work}

Our approach is basically composed of two components: \textit{generative modeling} and \textit{knowledge distillation}, which both have gained comprehensive attention in the deep learning community in recent years.

% =================================================================================
% Generative Image Modeling
% =================================================================================
\textbf{Generative Image Modeling.}

With Generative Adversarial Networks (GANs) \cite{Goodfellow2014GAN} at forefront of modeling image generation, a series of studies on GANs and its variants \cite{Brock2019BigGAN}\needcite{other GAN papers} have shown great potential of generating high-fidelity synthetic images with generator models learned from training data.
One appealing prospective application of synthetic image generation is data augmentation.
Recent studies have employed GAN-based augmentation to improve the model performance in data-restricted scenarios such as medical imaging \cite{Frid2018GANMedImageAug,Han2019GANMedImageAug}.
However, this has never worked in practice on large-scale data yet as stated by \citet{Goodfellow2019AAAITalk}, and \notsure{a more extreme practice of training only} on GAN-synthesized data would lead to huge performance degradation \notsure{when compared with training on the original one} \cite{Yin2020DeepInversion} \needcite{others?}.
Another minority lane of image synthesis comes from the by-product of researches on reversible networks \cite{Behrmann2019iResNet,Gomez2017RevNet,Jacobsen2018iRevNet}.
These works propose a kind of reversible models where each layer's activations can be reconstructed from the next layer's.
The initial motivation is to save memory by computing the activations on-the-fly during backpropagation, while some researchers also find it useful to \notsure{train on a reversible problem} of imaging and use the reversed model for generation \cite{Asim2020iVNetDenoise}. \todo{need example}
Though adept at generating high-quality images, all aforementioned methods require access to the original data.

% =================================================================================
% Knowledge Distillation
% =================================================================================
\textbf{Knowledge Distillation.}
Knowledge distillation is a compression technique in which a compact model - the \textit{student} - is trained under the guidance of a larger model - the \textit{teacher} - or an ensemble of models. In a typical image classification task, the logits, e.g., the output of last layer in a deep neural network, are used as the carriers of the knowledge from the teacher model, which is not explicitly provided by the training set.
In principle, a model performing well on the training set will predict an output distribution with high probability on the correct class and with near-zero probabilities on other classes. Some of these ``non-zero'' probabilities are larger than others and reflect, to some extent, the generalization capabilities of the model and how well it will perform on the test set.
There have been various variations of knowledge distillation in terms of knowledge type and distillation strategies. One direction is to transfer additional knowledge in the form of intermediate activations \cite{romero2014fitnets,aguilar2020knowledge,zhang2017knowledge}, attention maps \cite{zagoruyko2016paying}, weight projections \cite{lee2018self} or layer interactions \cite{yim2017gift}. Other methods try to directly address the capacity gap between a teacher and student by distilling from a series of intermediate teachers \cite{mirzadeh2020improved,jin2019knowledge}. \todo{comments?}

% =================================================================================
% Data-Free Model Compression
% =================================================================================
\textbf{Data-Free Model Compression.}
Model compression in the context where the original data is not available has attracted growing interest in privacy-sensitive and data-restricted scenarios.
Methods in this setting essentially resort to synthetic image generation.
\needcite{Lopes} first attempt to pre-store activation statistics of each layer from the teacher model and build synthetic inputs that produces similar activations.
Follow-up works \needcite{} have developed the approach by using less meta-data or proposing different optimization objectives to match them.
These methods typically obtain the synthetic inputs by directly optimizing some trainable random noise with regards to a pre-determined objective, which is costly and time-consuming to produce sufficient data for compression.
There are also a few methods that synthesize input data via generative image modeling \needcite{}, which create substitute data much more efficiently than optimizing input noise.
However, scaling to tasks with large dataset, \eg ImageNet classification, remains challenging for these methods.

Our work follows the track of generative image modeling to attain efficient data generation, and \notsure{is the first that can successfully be applied to ImageNet to the best of our knowledge.}

